On the Complexity of Checking Transactional Consistency

Transactions simplify concurrent programming by enabling computations on shared data that are isolated from other concurrent computations and are resilient to failures. Modern databases provide different consistency models for transactions corresponding to different tradeoffs between consistency and availability. In this work, we investigate the problem of checking whether a given execution of a transactional database adheres to some consistency model. We show that consistency models like read committed, read atomic, and causal consistency are polynomial time checkable while prefix consistency and snapshot isolation are NP-complete in general. These results complement a previous NP-completeness result concerning serializability. Moreover, in the context of NP-complete consistency models, we devise algorithms that are polynomial time assuming that certain parameters in the input executions, e.g., the number of sessions, are fixed. We evaluate the scalability of these algorithms in the context of several production databases.

==> ser_dfs_fig.tex <==
%!TEX root = draft.tex

\tikzset{
 ser_history/.pic={
   \node[draw, rounded corners=2mm, minimum width=6.5cm, minimum height=3.5cm] (-box) at (0, 0) {};
   \node[draw, rounded corners=2mm] (-t1) at (0, 1.2) {\begin{tabular}{l} \texttt{x = 0;} \end{tabular}};
   \node[draw, rounded corners=2mm] (-t2r) at (-1.6, 0) {\begin{tabular}{l} \texttt{read(x); // 0} \end{tabular}};
   \node[draw, rounded corners=2mm] (-t2w) at (-1.6, -1.2) {\begin{tabular}{l}  \texttt{x = 1;} \end{tabular}};
   \node[draw, rounded corners=2mm] (-t3r) at (1.6, 0) {\begin{tabular}{l} \texttt{read(x); // 0} \end{tabular}};
   \node[draw, rounded corners=2mm] (-t3w) at (1.6, -1.2) {\begin{tabular}{l} \texttt{x = 2;} \end{tabular}};
   \path [name prefix ..] (#1-t2r) edge node[pos=0.5] {$\so$} (#1-t2w);
   \path [name prefix ..] (#1-t3r) edge node[pos=0.5] {$\so$} (#1-t3w);
   \path [name prefix ..] (#1-t1) edge node[left, pos=0.5] {$\so$} (#1-t2r);
   \path [name prefix ..] (#1-t1) edge node[pos=0.5] {$\so$} (#1-t3r);
  }
}

\begin{figure}

 \begin{subfigure}{.44\textwidth}
  \resizebox{\textwidth}{!}{
   \begin{tikzpicture}[->,>=stealth',shorten >=1pt,auto,node distance=3cm,
     semithick, transform shape]
    \pic (v00) at (0, 0)    {ser_history=v00};
    \pic (v10) at (-3.5, -4)    {ser_history=v10};
    \pic (v20) at (-7, -8)    {ser_history=v20};
    \pic (v11) at (0, -8)    {ser_history=v11};
    \pic (v21) at (-3.5, -12)    {ser_history=v21};
    \pic (v22) at (0, -16)    {ser_history=v22};
    \path (v00-box) edge[blue] node {} (v10-box); 
    \path (v10-box) edge[red] node {} (v20-box); 
    \path (v10-box) edge[blue] node {} (v11-box); 
    \path (v11-box) edge[blue] node {} (v21-box); 
    \path (v21-box) edge[blue] node {} (v22-box);
    
    % \draw[-, blue, dashed] plot[smooth, tension=2] coordinates { (-1.5,1.5) (0, .5) (1.5, 1.5)};
    \draw[-, blue, dashed] plot coordinates { (-1.2,1.7) (-1.2, .7) (1.2, .7) (1.2, 1.7)};
    \draw[-, blue, dashed] plot coordinates { (-7,-2.3) (-7,-4.5) (-3.5,-4.5) (-3.5,-3.5) (-1.5,-3.5) (-1.5,-2.3) };
    \draw[-, blue, dashed] plot coordinates { (-3.5,-6.3) (-3.5,-8.5) (3.4,-8.5) (3.4,-6.3) };
    % \draw[-, blue, dashed] plot coordinates { (-10.5,-6.5) (-10.5,-10) (-7, -10) (-7, -7.5) (-3.6,-7.5) (-3.6,-6.5) };
    \draw[-, blue, dashed] plot coordinates { (-10.5,-6.3) (-10.5,-8.5) };
    \draw[-, red, dashed] plot coordinates { (-10.5,-8.5) (-10.5,-10) (-7,-10) (-7, -8.5) };
    \draw[-, blue, dashed] plot coordinates { (-7, -8.5) (-7, -7.5) (-3.6,-7.5) (-3.6,-6.3) };
    \draw[-, blue, dashed] plot coordinates { (-7,-10.3) (-7,-14) (-3.5, -14) (-3.5, -12.5) (-.1,-12.5) (-.1,-10.3) };
    \draw[-, blue, dashed] plot coordinates { (-3.5,-14.3) (-3.5,-17.9) (3.4, -17.9) (3.4,-14.3) };
    % \draw[-, blue, dashed] plot coordinates { (-10.5,-6.5) (-10.5,-8.5) (-3.5,-8.5) (-3.5,-6.5) };
    
   \end{tikzpicture}  
  }
  \caption{Depth first search for serializable order. Red arrow implies the DFS is blocked, blue arrow implies the DFS went through.}
  \label{ser_algo_example:3}
 \end{subfigure}
 \caption{}
 \label{}
\end{figure}


==> ser_prefix.tex <==
%!TEX root = draft.tex

Without loss of generality, we will assume $\wro \cup \so$ is acyclic. Because cycles in $\wro \cup \so$ can be detected by simple polynomial graph search algorithm. Presence of cycles in $\wro \cup \so$ will imply there is no total order extending $\wro \cup \so$. 

